Core Challenges in Embodied Vision-Language Planning

Recent advances in the areas of multimodal machine learning and artificial intelligence (AI) have led to the development of challenging tasks at the intersection of Computer Vision, Natural Language Processing, and Embodied AI. Whereas many approaches and previous survey pursuits have characterised one or two of these dimensions, there has not been a holistic analysis at the center of all three. Moreover, even when combinations of these topics are considered, more focus is placed on describing, e.g., current architectural methods, as opposed to also illustrating high-level challenges and opportunities for the field. In this survey paper, we discuss Embodied Vision-Language Planning (EVLP) tasks, a family of prominent embodied navigation and manipulation problems that jointly use computer vision and natural language. We propose a taxonomy to unify these tasks and provide an in-depth analysis and comparison of the new and current algorithmic approaches, metrics, simulated environments, as well as the datasets used for EVLP tasks. Finally, we present the core challenges that we believe new EVLP works should seek to address, and we advocate for task construction that enables model generalizability and furthers real-world deployment.

==> tables/dataset_env.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Dataset      & \begin{tabular}[c]{@{}l@{}}Simulated\\ Real\end{tabular} & \begin{tabular}[c]{@{}l@{}}Indoors(I) \\ Outdoors (O)\end{tabular} & Modalities & Scale                      & Environments                                      \\ \hline
DeepMind Lab & S                                                        & O                                                                  &            & Few mazes                  & DeepMind Lab                                      \\ \hline
AI2-THOR     & S/R                                                      & I                                                                  &            & 32 Rooms                   & AI2-THOR                                          \\ \hline
VizDoom      & S                                                        & O                                                                  &            & Few Mazes                  & VizDoom                                           \\ \hline
Gibson       & S/R                                                      & I                                                                  &            & 572 buildingsm 1400 floors & Gibson, AI Habitat                                \\ \hline
Replica      & R                                                        & I                                                                  &            &                            & AI Habitat                                        \\ \hline
SUNCG        & S                                                        & I                                                                  &            & 45k houses with 750k rooms & MINOS, Home3D, HoME                               \\ \hline
2D-3DS       & R                                                        & I                                                                  &            &                            & Gibson                                            \\ \hline
CARLA        & S                                                        & O                                                                  &            &                            & CARLA                                             \\ \hline
Matterport3D & R                                                        & I                                                                  &            & 90 buildings               & AI Habitat, MINOS, Matterport3D Simulator, Gibson \\ \hline
CHALET       & S                                                        & i                                                                  &            & 10 houses, 58 rookms       & CHALET                                            \\ \hline
RoboTHOR     & S/R                                                      & I                                                                  &            & 89 apartments              & RoboTHOR                                          \\ \hline
\end{tabular}
}
\end{table}

==> tables/env_modalities.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
Environment      & Agent                 & Modalities                                        & Baselines       \\ \hline
AI Habitat       & Continuous / Discrete & Multimodal                                        & RL, SLAM        \\ \hline
CARLA            & Continuous            & Multimodal                                        & RL, IL, Classic \\ \hline
CHALET           & Continuous            & RGB                                               &                 \\ \hline
Gibson Env       & Continuous / Discrete & RGB, Depth, Semantic Segmentations                & RL, Classic     \\ \hline
iGibson          & Continuous            & Multimodal                                        & RL              \\ \hline
MINOS            & Continuous / Discrete & Multimodal                                        & RL              \\ \hline
HoME             & Continuous            & RGB, Depth, Semantic Segmentations                &                 \\ \hline
Matterport3D     & Discrete              & RGB, Depth, Semantic Segmentation                 & IL              \\ \hline
Home3D           & Continuous            & RGB, Depth, Semantic Segmentations, Top-down maps & RL              \\ \hline
AI2-THOR (iTHOR) & Continuous / Discrete & Color                                             &                 \\ \hline
RoboTHOR         & Continuous            & RGB, Depth, Object semantics                      & RL              \\ \hline
DeepMind Lab     & Continuous            & RGB, Depth                                        & RL              \\ \hline
VizDoom          & Continuous            & RGB, Depth, Semantic Segmentations                & RL              \\ \hline
\end{tabular}
\label{Tab:SimModalities}
}
\caption{}
\end{table}

==> tables/sim_comparison.tex <==
% \begin{table}[ht]
% \caption{Comparison of simulation environments.}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c c c c c c c c c c c}
% \toprule
% \textbf{Environment} & \begin{tabular}[c]{@{}c@{}}\textbf{Indoors} /\\ \textbf{Outdoors}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Real} / \\ \textbf{Simulated}\end{tabular} & \textbf{Physics} & \textbf{Customizable} & \textbf{Sim2real} & \textbf{Navigation} & \begin{tabular}[c]{@{}c@{}}\textbf{Object} \\ \textbf{Interaction}\end{tabular} & \textbf{Language} & \begin{tabular}[c]{@{}c@{}}\textbf{Multi-}\\ \textbf{agent}\end{tabular} \\ \midrule
% AI Habitat   & in & real  & \textbullet   & \textbullet  & & \textbullet & & \textbullet & \\ 
% \hline
% AI2-THOR  & in & R/S   & \textbullet   & \textbullet  & \textbullet & \textbullet & \textbullet & \textbullet & \textbullet \\ 
% % \hline
% % RoboTHOR  & in & R/S   & \textbullet   &  & \textbullet & \textbullet & & & \\ 
% \hline
% Gibson Env   & in & R/S   & \textbullet   &  & \textbullet & \textbullet & & & \\
% \hline
% iGibson   & in & R/S   & \textbullet   &  & & \textbullet & \textbullet & & \textbullet \\
% \hline
% CHALET & in & sim.  & &  & & \textbullet & \textbullet & \textbullet & \\
% \hline
% MINOS  & out & R/S   & & \textbullet  & & \textbullet & & & \\
% \hline
% CARLA  & out & sim.  & &  & \textbullet & \textbullet & & & \\
% \hline
% HoME & in & sim.  & \textbullet   & \textbullet  & & \textbullet & & \textbullet  & \textbullet \\
% \hline
% Matterport3D & in & real  & &  & & \textbullet & & \textbullet & \\
% \hline
% Home3D & in & sim.  & &  & & \textbullet & & \textbullet & \\
% \hline
% ViZDoom   & out & sim.  & &  & & \textbullet & & & \\
% \hline
% DeepMind Lab & out & sim.  & & \textbullet  & & \textbullet & & & \\ \bottomrule
% \end{tabular}
% }
% \label{Tab:SimComp}
% \end{table}

\begin{table}[ht]
\footnotesize
\rowcolors{2}{gray!10}{white}
\caption{Comparison of simulation environments.}
\label{Tab:SimComp}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c c c c c c c c c}
\toprule
\textbf{Environment} & \begin{tabular}[c]{@{}c@{}}\textbf{Indoors} /\\ \textbf{Outdoors}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Real} / \\
\textbf{Simulated}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Navigation}\end{tabular} & \textbf{Physics} & \textbf{Customizable} & \textbf{Sim2real}  & \begin{tabular}[c]{@{}c@{}}\textbf{Object} \\ \textbf{Interaction}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Multi-}\\ \textbf{agent}\end{tabular} \\ \midrule
AI Habitat   & in & R & Continuous & \textbullet   & \textbullet  & & & \\

AI2-THOR  & in & R/S & continuous / discrete & \textbullet   & \textbullet  & \textbullet & \textbullet & \textbullet \\ 

% RoboTHOR  & in & R/S   & \textbullet   &  & \textbullet & \textbullet & & & \\ 

Gibson Env   & in & R/S   & \textbullet   &  & \textbullet & \textbullet & & & \\

% iGibson   & in & R/S   & \textbullet   &  & & \textbullet & \textbullet & & \textbullet \\

CHALET & in & S & / & &  & & \textbullet & \\

MINOS  & out & R/S & / & & \textbullet  & & & \\

% CARLA  & out & sim.  & &  & \textbullet & \textbullet & & & \\

HoME & in & S & / & \textbullet   & \textbullet  & & & \textbullet \\

Matterport3D & in & R & discrete & &  & & & \\

House3D & in & S & continuous  & &  & & & \\

% ViZDoom   & out & sim.  & &  & & \textbullet & & & \\

% DeepMind Lab & out & sim.  & & \textbullet  & & \textbullet & & & \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/sim_task.tex <==
\begin{table}[ht]
\rowcolors{2}{gray!10}{white}
\caption{Simulation environments comparison.}
\resizebox{\columnwidth}{!}{
\centering
\begin{tabular}{l c c c c c c c c} 
    \toprule
    \textbf{Environment} & 
    \textbf{Tasks} & 
    \begin{tabular}[c]{@{}@{}c@{}}
        \textbf{Navigation} \\ \scriptsize{\textbf{Continuous} / \textbf{Discrete}}
    \end{tabular} & 
    \begin{tabular}[c]{@{}@{}c@{}}
        \textbf{Environment} \\ \scriptsize{\textbf{Photorealistic} /  \textbf{Synthetic}}
    \end{tabular} &
    \begin{tabular}[c]{@{}c@{}}
        \textbf{Setting} \\ \scriptsize{\textbf{Indoors} /  \textbf{Outdoors}}
    \end{tabular} &
    \textbf{Large-Scale} &
    \textbf{Dialogue} &
    \textbf{Multi-Agent}  \\

 \midrule
 Matterport3DSim \textcite{Matterport3D} & VLN, VDHN, EOR      & Discrete     & Photorealistic & In & \cmark & & \\
 Habitat AI \textcite{AIHabitat}     & VLN, EQA       & Both  & Both  & In   & \cmark & & \\
 MINOS \textcite{MINOS}     &  EQA       & Both   & Both           & In & \cmark & & \\
 AI2-THOR \textcite{AI2THOR}        & VDHN, EQA, EGM & Both   & Synthetic      & In  & & \cmark & \cmark \\
%  MINOS           & VDHN           & Continuous   & Both           & In  & \\
 House3D \textcite{wu2018building}         & EQA            & Discrete   & Synthetic      & In  & \cmark & & \\
%  HoME            & EQA            & Continuous   & Simulated      & In   \\
%  CHALET          & EOR            & Continuous   & Synthetic      & In  %  & & &\\
 CerealBar \textcite{CerealBar}       & EGM            & Discrete & Synthetic      & Out  & & \cmark & \cmark \\
%  CHAI            & EGM            & Continuous   & Synthetic      & In   & & \\
 ArraMon \textcite{ArraMon}         & EGM            & Discrete   & Synthetic      & Out  & & \cmark & \\
 StreetLearn \textcite{mirowski2019learning}     & VLN, EOR            & Discrete   & Photorealistic & Out & \cmark &  & \\
% REVERIE          & EOR            & Discrete   & Photorealistic      & In   & & &\\
 \bottomrule
 \end{tabular}
 \label{Tab:SimTask}
}
\end{table}


==> tables/supervised_learning_models.tex <==
\begin{table}[ht]
\caption{Supervised learning approaches to improve \evlp tasks. Table comparing different supervised learning based approaches on VLN}
\label{tab:supervised_tasks}
\centering
 \begin{tabular}{l l l l l l} 
 \toprule
 \textbf{Method} & \textbf{Approach Type} & \textbf{SPL} & \textbf{SR} & \textbf{NE}  & \textbf{OSR} \\
\midrule
Speaker Follower & Data Augmentation & SPL & SR & NE  & OSR \\
Env Dropout & Data Augmentation & SPL & SR & NE  & OSR \\
Env Dropout & Data Augmentation & SPL & SR & NE  & OSR \\
Method & Approach Type & SPL & SR & NE  & OSR \\
 \bottomrule
 \end{tabular}
\end{table}

% For each paper add the reported scores on both the seen and unseen validation sets. Test sets too? Or are those only online and not available in the paper..
